$\infty$-Brush: Controllable Large Image Synthesis with Diffusion Models in Infinite Dimensions

Synthesizing high-resolution images from intricate, domain-specific information remains a significant challenge in generative modeling, particularly for applications in large-image domains such as digital histopathology and remote sensing. Existing methods face critical limitations: conditional diffusion models in pixel or latent space cannot exceed the resolution on which they were trained without losing fidelity, and computational demands increase significantly for larger image sizes. Patch-based methods offer computational efficiency but fail to capture long-range spatial relationships due to their overreliance on local information. In this paper, we introduce a novel conditional diffusion model in infinite dimensions, $\infty$-Brush for controllable large image synthesis. We propose a cross-attention neural operator to enable conditioning in function space. Our model overcomes the constraints of traditional finite-dimensional diffusion models and patch-based methods, offering scalability and superior capability in preserving global image structures while maintaining fine details. To our best knowledge, $\infty$-Brush is the first conditional diffusion model in function space, that can controllably synthesize images at arbitrary resolutions of up to $4096\times4096$ pixels. The code is available at https://github.com/cvlab-stonybrook/infinity-brush.

==> tables/augment.tex <==
{
\centering
\begin{subtable}[t]{0.48\columnwidth}{
\centering
\resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|c|}
    \hline
    Method   & Embedding similarity          \\ 
    \hline
    Patch-based [10]             & 0.924              \\ 
    
    \texttt{$\infty$-Brush}        &  \textbf{0.947}           \\ 
    
    \hline
    \end{tabular}}
\caption{Embedding similarity between real and synthetic images on BRCA}
    \label{tab:bach}
}
\end{subtable}
\hfill
\begin{subtable}[t]{0.48\columnwidth}{
    \centering
\resizebox{1\linewidth}{!}{
    \begin{tabular}{|c|c|}
    \hline
    Training Data       & Test Acc         \\ 
    \hline
    Real             & 79 \%            \\ 
    Real + synthetic & \textbf{83 \%}  \\ 
    \hline
    \end{tabular}}
    \caption{Synthetic data improves accuracy drastically on BACH test set.}
    \label{tab:nct-crc}
}
\end{subtable}
}
